Effect of stellar rotation on the development of post-shock instabilities during core-collapse supernovae

The growth of instabilities is key to trigger a supernova explosion during the phase of stalled shock, immediately after the birth of a proto-neutron star (PNS). We assess the effect of stellar rotation on neutrino-driven convection and SASI when neutrino heating is taken into account. Rotation affects the frequency of the mode m=2 detectable with gravitational waves (GW). We use a linear stability analysis in the equatorial plane between the PNS and the stationary shock and consider a large range of specific angular momenta, neutrino luminosities and mass accretion rates. The nature of the dominant instability depends on the convection parameter chi and the rotation rate. Convective modes with chi>=5 are hampered by differential rotation. At smaller chi, however, mixed SASI-convective modes with a large angular scale m=1,2,3 benefit from rotation and become dominant for relatively low rotation rates at which centrifugal effects are small. For rotation rates >0.3 Keplerian rotation at the PNS surface (KPNS), the growth rate of the dominant mode depends weakly on neutrino heating which highlights a new instability regime. Its frequency is surprisingly independent of the heating rate, with a strong prograde spiral m=2 dominating over a large parameter range, favourable to the production of GW. A simple linear relation exists between the dominant oscillation frequency and the specific angular momentum. Three regimes are distinguished. For rotation rates <0.1KPNS, differential rotation has a quadratic effect on equatorial purely convective modes and a linear destabilizing effect on SASI. Intermediate rotation rates (0.1 to 0.3KPNS) lead to the emergence of mixed SASI/convection/rotation modes involving large angular scales. Finally, strong rotation erases the influence of buoyancy on the instability. This allows for a reduction of the parameter space, which is valuable for GW analysis.

==> Stellar rotation and the convective instability (Anne-Cécile)/part_mixed_modes_before.tex <==
\subsubsection{Mixed SASI-convective mode induced by rotation}

For intermediate rotation rates ($0.1<j<0.3$), the behaviour of the modes is modified by rotation to such an extent that it becomes impossible to distinguish clearly between convective and SASI modes. As will be described in this section, the modes in this regime retain characteristics of both instabilities and should be understood as mixed SASI/convection/rotation modes. 

\begin{figure*}[h]
    \centering
    \includegraphics[width=\hsize]{rsh5_pictures/structure_rsh5-10p.png}
    \caption{Spatial structure of the eigenmode entropy perturbation in the equatorial plane, for $\varepsilon=0.3$ and $\chi\sim6$. Each row corresponds to a value of $m=(1,2,4,5)$ (from top to bottom) and each column to a rotation rate with $j=(0,0.1,0.4)$ (from left to right). In magenta and cyan, we represented the gain and corotation radii, respectively. The diagonal sequence of framed plots corresponds to the most unstable modes. Coordinates $x$ and $y$ are expressed in $r_{\rm PNS}$ unit. The deformation induced by rotation is stronger for smaller scale modes.}
    \label{structure}
\end{figure*}

%Jolies images
In order to gain a deeper understanding of the transition between the SASI dominated and the buoyancy dominated mode including rotation, we show in Fig.~\ref{structure} the entropy structure of the eigenfunction for the modes $m=1,2,4,5$ for three values of the angular momentum $j=0$, $0.1$ and $0.4$ and $\chi\sim 6$. When there is no rotation (first column in Fig.~\ref{structure}), the entropy structure of SASI (first line) uniformly spread in the radial direction as a spiral pattern is clearly distinct from the structure of convection, whose perturbations are more localised in the vicinity of the gain radius and do not display any spiral pattern. In the second column of this figure, we note that the $m=1$ spiral SASI pattern is little affected by the rotation (compare left and middle columns). This can be interpreted by the fact that for such moderate rotation, the corotation radius is close to the PNS surface. For the same rotation rate, the differential rotation shears the convective cells with $m=2-5$. This leads to spiral structures that are smaller but similar to a SASI pattern. However, the convective nature of the mode is still visible by the localisation of perturbations near the gain radius. These similar structures can be explained if we consider that the mode is not purely convective, but becomes a mixed mode SASI/convection/rotation.

\begin{figure*}[htbp]
    \centering
    %\hspace{-6.cm}
    %\includegraphics[width=\hsize]{rsh5_pictures/Pano_eps0-05.png}%pano_varEps.png}
    \includegraphics[width=0.72\textwidth]{rsh5_pictures/pano-5.png}
    \caption{From left to right, maps of the growth rate $\omega_i$, frequency $\omega_r$, azimuthal number $m$ and corotation radius of the most unstable fundamental mode with three dissociation rates $\varepsilon=0$ (top row), $0.3$ (middle row) and $0.5$ (bottom row). Above the magenta dashed line, the growth rate of equatorial perturbations decreases with rotation. In the two left columns, the white lines show where the corotation radius equals $r_{\rm PNS}$ and $r_{\rm gain}$. In the two right columns, the black lines highlight the variation of the dominant azimuthal number $m$ (numbers).}
    \label{pano}
\end{figure*}

A global panorama of the parameter space is shown in Fig.~\ref{pano} where we vary $\chi$ and $j$ for three values of the dissociation parameter $\varepsilon=0$, $0.3$ and $0.5$ (upper to lower rows). The four columns represent the growth rate and oscillation frequency of the most unstable mode, its azimuthal number $m$ and the corotation radius $r_{\rm corot}$. The main effect of dissociation is to diminish the radius of the stationary shock and thus the size of the gain region and the timescale of advection.

%variation frequence
For small values of $j$, we can see a sharp jump in frequency and $m$ when neutrino heating exceeds the threshold $\chi\sim 4$ corresponding to the transition from SASI to the convective instability as the most unstable mode. As angular momentum is increased above $j_{\rm crit}\sim 0.08-0.12$, however, this jump disappears and it becomes impossible to distinguish clearly convective and SASI modes. 

The first column in Fig.~\ref{pano} shows the adverse effect of rotation on the growth rate of the convective instability for $\chi>5$, as discussed in Sect.~\ref{sec:convection_rotation}. For each rotation rate, the magenta line highlights the value of $\chi$ above which the rotation has an adverse effect on the growth of convection in the equatorial plane. In this region, the dynamic of the flow will be dominated by axisymmetric modes that are expected to be little affected by the rotation for $j\in[0,0.5]$. This stands in contrast with the beneficial effect on the growth rate of SASI for $\chi<3-4$, as discussed in Sect.~\ref{sec:sasi_rotation}, where spiral modes are therefore expected to dominate the dynamics.
%The rotational stabilisation of equatorial convection observed in the simulations of \cite{FryerHeger2000} and \cite{FryerWarren2004} is also supported by the left plot in Fig.~\ref{rot_effect_conv}, where the damping effect is more pronounced for the modes with a smaller angular scale $m=4$ compared to $m=2$. 
 Interestingly, rotation has a beneficial effect on the growth rate of the dominant non-axisymmetric convective modes for moderate convection parameters $\chi \simeq 4-5$. The same behaviour can be observed for the $m=4$ mode in the upper plot of Fig.~\ref{wi(chi)_rot}, where the growth rate for $\chi\sim 3-4$ is significantly enhanced by rotation. It is also linked to the easier onset of convection with rotation shown by the decrease of $\chi_{\rm marg}$ in Fig.~\ref{chi_crit(j)_varm}, as discussed in Sect.~\ref{sec:convection_rotation}. All these observations can be interpreted if the perturbation of the shock induced by the convective instability produced an advective acoustic cycle favourable to enhance the convective instability, as already suggested by the entropy structure in Fig.~\ref{structure}. 
The mode $m=1$ in Fig.~\ref{rot_effect_conv} calls for a particular attention, with a significant enhancement of the growth rate by rotation  (this is also true for the $m=2$ mode in the lower panel of the same figure) in a regime $\chi=6.5$ a priori dominated by convection with an adverse effect of rotation. This peculiar behaviour of the $m=1-2$ modes can also be explained by a mixed state of this mode with the advective-acoustic cycle interacting constructively with the convective mode. Indeed, for these low values of $m$ the transition from SASI to convection takes place at a rather large value of $\chi$ (e.g. $\chi \simeq 6$ for $m=1$ in Fig.~\ref{wi(chi)}). As a consequence, mixed modes with a beneficial effect of rotation may be expected for larger values of $\chi$ close to this transition.

 %The same applies to the intermediate region $\chi\sim5$ in Fig.~\ref{pano}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{rsh5_pictures/mi_evol_wi_wr(j)_eps00chi45.png}
    \caption{Growth rate (top) and frequency (bottom) evolution of several modes depending on the rotation rate $j$, for $\chi=4.5$, $\varepsilon=0$ and $r_{\rm sh}(j=0)=6.8r_{\rm PNS}$.}
    \label{evol_wi}
\end{figure}

%variation du $m$ dominant

We remark in the 3rd column of Fig.~\ref{pano} that the azimuthal number $m$ of the most unstable mode decreases with the rotation rate for $\chi>4$, while it increases for $\chi<4$. The change of dominant convective scale induced by rotation is not predicted by Eq.~\eqref{eq_m}: comparing the magenta and blue triangles in Fig.~\ref{m_dom(eps)} indicates a shift to larger angular scales induced by a moderate angular momentum $j=0.08$, despite a negligible change in the size of the gain region. For this small rotation rate, the shortcoming of Eq.~\eqref{eq_m} is not surprising when considering the rotation-induced distortion of the convective cells in Fig.~\ref{structure} and the lingering influence of SASI. The rotational stabilisation of perturbations with a large azimuthal wave number $m$ can be understood as a consequence of their strong shear (Eq.~\ref{doppler_omega}) which induces a short radial wavelength $2\pi v/\omega'$ for advected perturbations near the PNS, and thus a phase mixing particularly visible in the lower right corner of Fig.~\ref{structure}. 

%-----Growth rate mixed modes


\begin{figure}[h]
    \centering
    %\includegraphics[width=\hsize]{rsh5_pictures/evol_wi(j)_eps06.png} %06 --> simplement indice de la figure, pas = à eps ici mais oui pour les deux figures suivantes
    \includegraphics[width=\columnwidth]{rsh5_pictures/mi_evol_wi_wr(j)_eps09chi45.png}
    \caption{Same as Fig.~\ref{evol_wi} but for $\varepsilon=0.3$ and $r_{\rm sh}(j=0)=3.9r_{\rm PNS}$.}
    \label{evol_wi_dis}
\end{figure}


Figs.~\ref{evol_wi} and \ref{evol_wi_dis} illustrate the effect of rotation on both instabilities in two configurations mainly differing by their shock radius, induced by the dissociation parameter. The value $\chi=4.5$ is chosen in the region where the most unstable mode is convective and the growth rate increases with rotation (below the magenta line of the first column in Fig.\ref{pano}). 
In the bottom panel of these figures, we can differentiate the initially convective modes ($\omega_r(j=0)=0$) from the initially SASI modes ($\omega_r(j=0)\neq0$). We can see that the convective frequency, enhanced by rotation, is similar to the SASI frequency for $j\in[0.02,0.08]$. The top panels of this figure show that the effect of rotation varies depending on the nature of the instability. The growth rate of SASI modes is enhanced by the rotation, as in \cite{YamasakiFoglizzo2008} and \cite{Blondin+2017}. For convective modes, the effect of rotation depends on the proximity of $\chi$ to the transition value $\chi_{\rm trans}$ defining the transition of a mode between SASI and convection. Defining $\Delta \chi\equiv\chi-\chi_{\rm trans}$, the rotation can induce an increase of the growth rate, similar to the effect of rotation on SASI, if $\Delta \chi<1$. Otherwise, the convective modes are quenched by rotation, as observed in Fig.~\ref{rot_effect_conv}. %This is another indication of the mixed nature of the modes.
Comparing Figs.~\ref{evol_wi} and \ref{evol_wi_dis}, the increase of the frequency and growth rate induced by rotation is stronger for $\varepsilon=0.3$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{rsh5_pictures/wi(m)_varL_chifix40.png}
    \caption{Evolution of the growth rate depending on the azimuthal number $m$ for several rotation rates and $\chi=4.5$.}
    \label{wi(m)_varrot}
\end{figure}

Figure~\ref{wi(m)_varrot} illustrates the complexity of the impact of rotation depending on the azimuthal number. For initially SASI modes ($m=1,2$), the rotation increases the growth rate. However, for initially convective modes, the effect of rotation depends on both the rotation and the azimuthal number. For $m\sim3$, the destabilising effect of rotation on the convective instability can be clearly seen by continuity with the increase of the SASI growth rate. For $m \in [3,5]$, the effect of rotation on the convection is similar to its effect on SASI. 
For higher $m\gtrsim6$ and low rotation rates, the rotation has an adverse effect and leads to a decrease of the growth rate. The effect change for high rotation rates and will be discussed in Sect.~\ref{part:high_rot}.

Figure~\ref{rcorot_m2mdom} allows us to estimate the rotation rate above which these mixed modes appear. This threshold corresponds to the critical rotation rate above which the corotation radius starts to move away from the Brunt-V\"ais\"al\"a radius. We remark that $r_{\rm corot}$ starts to shift outwards for rotation rates exceeding $j\sim10\%$, indicating a lower frequency than expected for a purely convective mode with negligible advection. This slower oscillation frequency compared to the rotation rate of the most buoyant layer suggests that some physical process associated to rotation contributes significantly to the instability mechanism. The rotation threshold $j\sim10\%$ corresponds to an oscillation frequency of the convective mode comparable to the oscillation frequency of the spiral SASI mode, without heating nor rotation (magenta points of Fig.~\ref{jcrit(eps)}). However, the change of the size of the dominant scale keeps the corotation close to the Brunt-Väisälä radius, indicating that convection still plays a role in the instability mechanism. 

To better constrain the domain of existence of these mixed modes, we use the third column of Fig.~\ref{pano}. We can see that for small rotation rates, the azimuthal number limits converge to a line at $\chi\sim 4$. It corresponds to the transition from purely SASI modes to purely convective modes. Above this boundary, the high $m$ modes dominate, and their frequency depends linearly on the rotation rate. However, when we increase the rotation rates, one can see that this frontier disappears and the transition from small $m$ to higher $m$ is continuous. The value of the rotation rate $j_{\rm crit}$ when the frontier disappears slightly increases when the dissociation rate increases (blue points in Fig.~\ref{jcrit(eps)}). This behaviour is also found considering critical rotation rate at which the rotation frequency matches the frequency of the modes $m=4$ without rotation nor heating (magenta points of Fig.~\ref{jcrit(eps)}).
This is the signature of the growth of mixed modes SASI/convection/rotation.

\begin{figure}[h]
    \centering
    \includegraphics[width=\hsize]{rsh5_pictures/mi_jcrit(eps).png}
    \caption{Evolution of the critical rotation rate $j_{\rm crit}$ depending on the dissociation using two methods. This critical rotation corresponds to the apparition of the mixed-modes. The higher the dissociation, the later the transition. For the blue points, we used the discontinuity end of the dominant m at $\chi\sim4$. For the magenta points, we used the advection timescale $\tau_{\rm adv}$ from the shock to the gain radius for $m=4$ and $\chi\sim4$.}
    \label{jcrit(eps)}
\end{figure}

%These mixed modes exist until the rotation is so strong that it erases the effect of neutrino-heating. At this point, the instability is driven by rotation and not by buoyancy.

In the end, the rotation smoothened the transition from SASI to convection, leading to a mixed mode phase. These mixed modes appear when the corotation radius moves away from the Brunt-Väisälä radius and exist up to $j\sim30\%$ where the behaviour of the modes starts to change.% where the influence of neutrino-heating is negligible and the behaviours of the modes are driven by the rotation rate.



==> part_mixed_modes_before.tex <==
\subsubsection{Mixed SASI-convective mode induced by rotation}

For intermediate rotation rates ($0.1<j<0.3$), the behaviour of the modes is modified by rotation to such an extent that it becomes impossible to distinguish clearly between convective and SASI modes. As will be described in this section, the modes in this regime retain characteristics of both instabilities and should be understood as mixed SASI/convection/rotation modes. 

\begin{figure*}[h]
    \centering
    \includegraphics[width=\hsize]{rsh5_pictures/structure_rsh5-10p.png}
    \caption{Spatial structure of the eigenmode entropy perturbation in the equatorial plane, for $\varepsilon=0.3$ and $\chi\sim6$. Each row corresponds to a value of $m=(1,2,4,5)$ (from top to bottom) and each column to a rotation rate with $j=(0,0.1,0.4)$ (from left to right). In magenta and cyan, we represented the gain and corotation radii, respectively. The diagonal sequence of framed plots corresponds to the most unstable modes. Coordinates $x$ and $y$ are expressed in $r_{\rm PNS}$ unit. The deformation induced by rotation is stronger for smaller scale modes.}
    \label{structure}
\end{figure*}

%Jolies images
In order to gain a deeper understanding of the transition between the SASI dominated and the buoyancy dominated mode including rotation, we show in Fig.~\ref{structure} the entropy structure of the eigenfunction for the modes $m=1,2,4,5$ for three values of the angular momentum $j=0$, $0.1$ and $0.4$ and $\chi\sim 6$. When there is no rotation (first column in Fig.~\ref{structure}), the entropy structure of SASI (first line) uniformly spread in the radial direction as a spiral pattern is clearly distinct from the structure of convection, whose perturbations are more localised in the vicinity of the gain radius and do not display any spiral pattern. In the second column of this figure, we note that the $m=1$ spiral SASI pattern is little affected by the rotation (compare left and middle columns). This can be interpreted by the fact that for such moderate rotation, the corotation radius is close to the PNS surface. For the same rotation rate, the differential rotation shears the convective cells with $m=2-5$. This leads to spiral structures that are smaller but similar to a SASI pattern. However, the convective nature of the mode is still visible by the localisation of perturbations near the gain radius. These similar structures can be explained if we consider that the mode is not purely convective, but becomes a mixed mode SASI/convection/rotation.

\begin{figure*}[htbp]
    \centering
    %\hspace{-6.cm}
    %\includegraphics[width=\hsize]{rsh5_pictures/Pano_eps0-05.png}%pano_varEps.png}
    \includegraphics[width=0.72\textwidth]{rsh5_pictures/pano-5.png}
    \caption{From left to right, maps of the growth rate $\omega_i$, frequency $\omega_r$, azimuthal number $m$ and corotation radius of the most unstable fundamental mode with three dissociation rates $\varepsilon=0$ (top row), $0.3$ (middle row) and $0.5$ (bottom row). Above the magenta dashed line, the growth rate of equatorial perturbations decreases with rotation. In the two left columns, the white lines show where the corotation radius equals $r_{\rm PNS}$ and $r_{\rm gain}$. In the two right columns, the black lines highlight the variation of the dominant azimuthal number $m$ (numbers).}
    \label{pano}
\end{figure*}

A global panorama of the parameter space is shown in Fig.~\ref{pano} where we vary $\chi$ and $j$ for three values of the dissociation parameter $\varepsilon=0$, $0.3$ and $0.5$ (upper to lower rows). The four columns represent the growth rate and oscillation frequency of the most unstable mode, its azimuthal number $m$ and the corotation radius $r_{\rm corot}$. The main effect of dissociation is to diminish the radius of the stationary shock and thus the size of the gain region and the timescale of advection.

%variation frequence
For small values of $j$, we can see a sharp jump in frequency and $m$ when neutrino heating exceeds the threshold $\chi\sim 4$ corresponding to the transition from SASI to the convective instability as the most unstable mode. As angular momentum is increased above $j_{\rm crit}\sim 0.08-0.12$, however, this jump disappears and it becomes impossible to distinguish clearly convective and SASI modes. 

The first column in Fig.~\ref{pano} shows the adverse effect of rotation on the growth rate of the convective instability for $\chi>5$, as discussed in Sect.~\ref{sec:convection_rotation}. For each rotation rate, the magenta line highlights the value of $\chi$ above which the rotation has an adverse effect on the growth of convection in the equatorial plane. In this region, the dynamic of the flow will be dominated by axisymmetric modes that are expected to be little affected by the rotation for $j\in[0,0.5]$. This stands in contrast with the beneficial effect on the growth rate of SASI for $\chi<3-4$, as discussed in Sect.~\ref{sec:sasi_rotation}, where spiral modes are therefore expected to dominate the dynamics.
%The rotational stabilisation of equatorial convection observed in the simulations of \cite{FryerHeger2000} and \cite{FryerWarren2004} is also supported by the left plot in Fig.~\ref{rot_effect_conv}, where the damping effect is more pronounced for the modes with a smaller angular scale $m=4$ compared to $m=2$. 
 Interestingly, rotation has a beneficial effect on the growth rate of the dominant non-axisymmetric convective modes for moderate convection parameters $\chi \simeq 4-5$. The same behaviour can be observed for the $m=4$ mode in the upper plot of Fig.~\ref{wi(chi)_rot}, where the growth rate for $\chi\sim 3-4$ is significantly enhanced by rotation. It is also linked to the easier onset of convection with rotation shown by the decrease of $\chi_{\rm marg}$ in Fig.~\ref{chi_crit(j)_varm}, as discussed in Sect.~\ref{sec:convection_rotation}. All these observations can be interpreted if the perturbation of the shock induced by the convective instability produced an advective acoustic cycle favourable to enhance the convective instability, as already suggested by the entropy structure in Fig.~\ref{structure}. 
The mode $m=1$ in Fig.~\ref{rot_effect_conv} calls for a particular attention, with a significant enhancement of the growth rate by rotation  (this is also true for the $m=2$ mode in the lower panel of the same figure) in a regime $\chi=6.5$ a priori dominated by convection with an adverse effect of rotation. This peculiar behaviour of the $m=1-2$ modes can also be explained by a mixed state of this mode with the advective-acoustic cycle interacting constructively with the convective mode. Indeed, for these low values of $m$ the transition from SASI to convection takes place at a rather large value of $\chi$ (e.g. $\chi \simeq 6$ for $m=1$ in Fig.~\ref{wi(chi)}). As a consequence, mixed modes with a beneficial effect of rotation may be expected for larger values of $\chi$ close to this transition.

 %The same applies to the intermediate region $\chi\sim5$ in Fig.~\ref{pano}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{rsh5_pictures/mi_evol_wi_wr(j)_eps00chi45.png}
    \caption{Growth rate (top) and frequency (bottom) evolution of several modes depending on the rotation rate $j$, for $\chi=4.5$, $\varepsilon=0$ and $r_{\rm sh}(j=0)=6.8r_{\rm PNS}$.}
    \label{evol_wi}
\end{figure}

%variation du $m$ dominant

We remark in the 3rd column of Fig.~\ref{pano} that the azimuthal number $m$ of the most unstable mode decreases with the rotation rate for $\chi>4$, while it increases for $\chi<4$. The change of dominant convective scale induced by rotation is not predicted by Eq.~\eqref{eq_m}: comparing the magenta and blue triangles in Fig.~\ref{m_dom(eps)} indicates a shift to larger angular scales induced by a moderate angular momentum $j=0.08$, despite a negligible change in the size of the gain region. For this small rotation rate, the shortcoming of Eq.~\eqref{eq_m} is not surprising when considering the rotation-induced distortion of the convective cells in Fig.~\ref{structure} and the lingering influence of SASI. The rotational stabilisation of perturbations with a large azimuthal wave number $m$ can be understood as a consequence of their strong shear (Eq.~\ref{doppler_omega}) which induces a short radial wavelength $2\pi v/\omega'$ for advected perturbations near the PNS, and thus a phase mixing particularly visible in the lower right corner of Fig.~\ref{structure}. 

%-----Growth rate mixed modes


\begin{figure}[h]
    \centering
    %\includegraphics[width=\hsize]{rsh5_pictures/evol_wi(j)_eps06.png} %06 --> simplement indice de la figure, pas = à eps ici mais oui pour les deux figures suivantes
    \includegraphics[width=\columnwidth]{rsh5_pictures/mi_evol_wi_wr(j)_eps09chi45.png}
    \caption{Same as Fig.~\ref{evol_wi} but for $\varepsilon=0.3$ and $r_{\rm sh}(j=0)=3.9r_{\rm PNS}$.}
    \label{evol_wi_dis}
\end{figure}


Figs.~\ref{evol_wi} and \ref{evol_wi_dis} illustrate the effect of rotation on both instabilities in two configurations mainly differing by their shock radius, induced by the dissociation parameter. The value $\chi=4.5$ is chosen in the region where the most unstable mode is convective and the growth rate increases with rotation (below the magenta line of the first column in Fig.\ref{pano}). 
In the bottom panel of these figures, we can differentiate the initially convective modes ($\omega_r(j=0)=0$) from the initially SASI modes ($\omega_r(j=0)\neq0$). We can see that the convective frequency, enhanced by rotation, is similar to the SASI frequency for $j\in[0.02,0.08]$. The top panels of this figure show that the effect of rotation varies depending on the nature of the instability. The growth rate of SASI modes is enhanced by the rotation, as in \cite{YamasakiFoglizzo2008} and \cite{Blondin+2017}. For convective modes, the effect of rotation depends on the proximity of $\chi$ to the transition value $\chi_{\rm trans}$ defining the transition of a mode between SASI and convection. Defining $\Delta \chi\equiv\chi-\chi_{\rm trans}$, the rotation can induce an increase of the growth rate, similar to the effect of rotation on SASI, if $\Delta \chi<1$. Otherwise, the convective modes are quenched by rotation, as observed in Fig.~\ref{rot_effect_conv}. %This is another indication of the mixed nature of the modes.
Comparing Figs.~\ref{evol_wi} and \ref{evol_wi_dis}, the increase of the frequency and growth rate induced by rotation is stronger for $\varepsilon=0.3$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{rsh5_pictures/wi(m)_varL_chifix40.png}
    \caption{Evolution of the growth rate depending on the azimuthal number $m$ for several rotation rates and $\chi=4.5$.}
    \label{wi(m)_varrot}
\end{figure}

Figure~\ref{wi(m)_varrot} illustrates the complexity of the impact of rotation depending on the azimuthal number. For initially SASI modes ($m=1,2$), the rotation increases the growth rate. However, for initially convective modes, the effect of rotation depends on both the rotation and the azimuthal number. For $m\sim3$, the destabilising effect of rotation on the convective instability can be clearly seen by continuity with the increase of the SASI growth rate. For $m \in [3,5]$, the effect of rotation on the convection is similar to its effect on SASI. 
For higher $m\gtrsim6$ and low rotation rates, the rotation has an adverse effect and leads to a decrease of the growth rate. The effect change for high rotation rates and will be discussed in Sect.~\ref{part:high_rot}.

Figure~\ref{rcorot_m2mdom} allows us to estimate the rotation rate above which these mixed modes appear. This threshold corresponds to the critical rotation rate above which the corotation radius starts to move away from the Brunt-V\"ais\"al\"a radius. We remark that $r_{\rm corot}$ starts to shift outwards for rotation rates exceeding $j\sim10\%$, indicating a lower frequency than expected for a purely convective mode with negligible advection. This slower oscillation frequency compared to the rotation rate of the most buoyant layer suggests that some physical process associated to rotation contributes significantly to the instability mechanism. The rotation threshold $j\sim10\%$ corresponds to an oscillation frequency of the convective mode comparable to the oscillation frequency of the spiral SASI mode, without heating nor rotation (magenta points of Fig.~\ref{jcrit(eps)}). However, the change of the size of the dominant scale keeps the corotation close to the Brunt-Väisälä radius, indicating that convection still plays a role in the instability mechanism. 

To better constrain the domain of existence of these mixed modes, we use the third column of Fig.~\ref{pano}. We can see that for small rotation rates, the azimuthal number limits converge to a line at $\chi\sim 4$. It corresponds to the transition from purely SASI modes to purely convective modes. Above this boundary, the high $m$ modes dominate, and their frequency depends linearly on the rotation rate. However, when we increase the rotation rates, one can see that this frontier disappears and the transition from small $m$ to higher $m$ is continuous. The value of the rotation rate $j_{\rm crit}$ when the frontier disappears slightly increases when the dissociation rate increases (blue points in Fig.~\ref{jcrit(eps)}). This behaviour is also found considering critical rotation rate at which the rotation frequency matches the frequency of the modes $m=4$ without rotation nor heating (magenta points of Fig.~\ref{jcrit(eps)}).
This is the signature of the growth of mixed modes SASI/convection/rotation.

\begin{figure}[h]
    \centering
    \includegraphics[width=\hsize]{rsh5_pictures/mi_jcrit(eps).png}
    \caption{Evolution of the critical rotation rate $j_{\rm crit}$ depending on the dissociation using two methods. This critical rotation corresponds to the apparition of the mixed-modes. The higher the dissociation, the later the transition. For the blue points, we used the discontinuity end of the dominant m at $\chi\sim4$. For the magenta points, we used the advection timescale $\tau_{\rm adv}$ from the shock to the gain radius for $m=4$ and $\chi\sim4$.}
    \label{jcrit(eps)}
\end{figure}

%These mixed modes exist until the rotation is so strong that it erases the effect of neutrino-heating. At this point, the instability is driven by rotation and not by buoyancy.

In the end, the rotation smoothened the transition from SASI to convection, leading to a mixed mode phase. These mixed modes appear when the corotation radius moves away from the Brunt-Väisälä radius and exist up to $j\sim30\%$ where the behaviour of the modes starts to change.% where the influence of neutrino-heating is negligible and the behaviours of the modes are driven by the rotation rate.


